Incremental Cardinality Constraints for MaxSAT

Maximum Satisfiability (MaxSAT) is an optimization variant of the Boolean Satisfiability (SAT) problem. In general, MaxSAT algorithms perform a succession of SAT solver calls to reach an optimum solution making extensive use of cardinality constraints. Many of these algorithms are non-incremental in nature, i.e. at each iteration the formula is rebuilt and no knowledge is reused from one iteration to another. In this paper, we exploit the knowledge acquired across iterations using novel schemes to use cardinality constraints in an incremental fashion. We integrate these schemes with several MaxSAT algorithms. Our experimental results show a significant performance boost for these algo- rithms as compared to their non-incremental counterparts. These results suggest that incremental cardinality constraints could be beneficial for other constraint solving domains.

==> blocking-encoding.tex <==
\DontPrintSemicolon
\SetKwFunction{encodeCNF}{CNF}
\SetKwFunction{encode}{encodeCNF}
\SetVlineSkip{1pt}
\begin{algorithm}[!t]
  \small
  \tcp*[l]{encode cardinality to CNF with incremental blocking}
  %\KwIn{\encode($x_1 + \ldots + x_n \leq k, \mathcal A, \mathcal U$)}
  %\KwOut{CNF encoding to $x_1, \ldots, x_n \leq k$ with incremental blocking}
  $\mathcal U \gets \{ b' : b' \in \mathcal A\}$\;
  $\mathcal A \gets \neg b$\tcp*[r]{\footnotesize b is a new variable}
  $\{o_1, \ldots, o_n\} \gets \encodeCNF(x_1 + \ldots + x_n \leq k, b)$\tcp*[r]{CNF with blocking variable}
  \lFor{$i=k+1$ \emph{\KwTo} $n$}{$\mathcal A \gets \mathcal A \cup \neg o_i$\tcp*[f]{disable sums from $k+1$ to $n$}}
  %\caption{Encoding to CNF with incremental blocking}\label{alg:incremental-blocking}
  \caption{{\tt encodeCard}($x_1 + \ldots + x_n \leq k, \mathcal A, \mathcal U$)}\label{alg:incremental-blocking}
\end{algorithm}


==> cnf-encoding.tex <==
\DontPrintSemicolon
\SetKwFunction{encode}{encodeCNF}
\SetKwFunction{encodeCNF}{CNF}
\SetVlineSkip{1pt}
\begin{algorithm}[!t]
  \small
  \KwIn{\encode($x_1 + \ldots + x_n \leq k, \mathcal A, \mathcal U$)}
  \KwOut{CNF encoding to $x_1, \ldots, x_n \leq k$}
  $(\mathcal A, \mathcal U) \gets (\emptyset, \emptyset)$\;
  $<o_1, \ldots, o_n> \gets \encodeCNF(x_1 + \ldots + x_n \leq k)$\;
  \lFor{$i=k+1$ \emph{\KwTo} $n$}{$\mathcal U \gets \mathcal U \cup \neg o_i$\tcp*[f]{disable sums from $k+1$ to $n$}}
  \caption{Encoding to CNF}\label{alg:incremental-blocking}
\end{algorithm}


==> fu-malik-inc-text.tex <==
Incremental blocking can also be used for MaxSAT algorithms that do not 
update cardinality constraints but modify the formula at 
each iteration. For example, Fu-Malik algorithm (Algorithm~\ref{alg:fu-malik-orig}, section~\ref{sec:preliminaries}) 
can be enhanced with incremental blocking. Algorithm~\ref{alg:fu-malik-inc} shows 
the modifications to Fu-Malik algorithm to support incremental blocking.
%
The main differences between the incremental and non-incremental versions of 
Fu-Malik Algorithm are highlighted. %in Algorithm~\ref{alg:fu-malik-inc}.
%Algorithm~\ref{alg:fu-malik-inc} and Algorithm~\ref{alg:fu-malik-orig} 
%are in the relaxation of soft clauses. 
%
For each soft clause $\omega$ in the $\varphi_C$, Algorithm~\ref{alg:fu-malik-inc} copies 
$\omega$ into $\omega_R$ without blocking variables (line 10). Next, it adds a fresh blocking 
variable $b$ and a fresh relaxation variable $r$ to $\omega_R$ (line 10). 
The current soft clause $\omega_R$ is enabled by adding $\neg b$ to the set of assumptions, 
where $b$ is the blocking variable that occurs in $\omega_R$ (line 12). At the same time, 
the assumption $\neg b'$ is removed from the set of assumptions, where $b'$ is the blocking
variable that occurs in $\omega$ (line 12). Finally, the formula $\varphi$ is updated with the 
new clause $\omega_R$, and with the unit clause $b'$. Note that this unit clause 
disables $\omega$ from the formula since $\omega$ contains $b'$ and therefore is always satisfied.

\Omit{
For each soft clause $\omega$ in the 
unsatisfiable subformula, Algorithm~\ref{alg:fu-malik-inc} copies $\omega$ into $\omega_R$ without 
blocking variables (line 12). Next, it adds a fresh blocking variable $b$ and a 
fresh relaxation $r$ to $\omega_R$ (line 12). This step allows the previous soft clause to 
be replaced by a new soft clause. To disable $\omega$ the algorithm adds the 
blocking variable occurring in $\omega$ to the set of unit clauses (line 13). 
Next, the negation of the blocking variable in $\omega_R$ is added to the 
set of assumption variables to enable $\omega_R$ for the upcoming iterations. 
Finally, the formula $\varphi$ is updated with the new clause $\omega_R$. 
After all soft clauses have been relaxed, the at-most-one constraint is added 
over the relaxation variables as in the original algorithm. The difference is 
that now the algorithm also adds the set of unit clauses ($\mathcal U$) to 
 $\varphi$, which disables the soft clauses that occurred in $\varphi_C$ for upcoming 
 iterations (line 16).
}

The incremental version of Fu-Malik algorithm creates $k$ auxiliary clauses at each 
iteration, where $k$ is the number of soft clauses in the unsatisfiable subformula. 
%
However, the size of unsatisfiable subformulas tends to be small when compared 
to the total number of soft clauses. 
%
Note that the number of auxiliary clauses created by the incremental version 
of Fu-Malik is not as large as when the incremental blocking is directly applied to 
cardinality encodings. %Furthermore, the size of unsatisfiable subformulas tend to 
%be small when compared to the total number of soft clauses.


==> weak-encoding.tex <==
\DontPrintSemicolon
\SetKwFunction{encodeCNF}{CNF}
\SetKwFunction{encode}{encodeCNF}
\SetKwData{hasEncoding}{hasEncoding}
\SetVlineSkip{1pt}
\begin{algorithm}[!t]
  \small
  \tcp*[l]{encode cardinality to CNF with incremental weakening}
  $(\mathcal A, \mathcal U) \gets (\emptyset, \emptyset)$\;
  \If{{\bf not} \hasEncoding}{
  \tcp*[l]{If the encoding has not been built}
  $\{o_1, \ldots, o_n\} \gets \encodeCNF(x_1 + \ldots + x_n \leq k)$\tcp*[r]{build the encoding}
  }
  %\eIf{\hasEncoding}{
  %\tcp*[l]{If the encoding has already been built}
  %\lFor{$i=k+1$ \emph{\KwTo} $n$}{$\mathcal A \gets \mathcal A \cup \neg o_i$\tcp*[f]{updates the output variables}}
  %}{
  %
  \lFor{$i=k+1$ \emph{\KwTo} $n$}{$\mathcal A \gets \mathcal A \cup \neg o_i$\tcp*[f]{updates the output variables}}
  \caption{{\tt encodeCard}($x_1 + \ldots + x_n \leq k, \mathcal A, \mathcal U$)}\label{alg:incremental-weak}
\end{algorithm}
